Data Pipeline Quality: Influencing Factors, Root Causes of Data-related Issues, and Processing Problem Areas for Developers

Data pipelines are an integral part of various modern data-driven systems. However, despite their importance, they are often unreliable and deliver poor-quality data. A critical step toward improving this situation is a solid understanding of the aspects contributing to the quality of data pipelines. Therefore, this article first introduces a taxonomy of 41 factors that influence the ability of data pipelines to provide quality data. The taxonomy is based on a multivocal literature review and validated by eight interviews with experts from the data engineering domain. Data, infrastructure, life cycle management, development & deployment, and processing were found to be the main influencing themes. Second, we investigate the root causes of data-related issues, their location in data pipelines, and the main topics of data pipeline processing issues for developers by mining GitHub projects and Stack Overflow posts. We found data-related issues to be primarily caused by incorrect data types (33%), mainly occurring in the data cleaning stage of pipelines (35%). Data integration and ingestion tasks were found to be the most asked topics of developers, accounting for nearly half (47%) of all questions. Compatibility issues were found to be a separate problem area in addition to issues corresponding to the usual data pipeline processing areas (i.e., data loading, ingestion, integration, cleaning, and transformation). These findings suggest that future research efforts should focus on analyzing compatibility and data type issues in more depth and assisting developers in data integration and ingestion tasks. The proposed taxonomy is valuable to practitioners in the context of quality assurance activities and fosters future research into data pipeline quality.

==> tables/tab-general_factors_all.tex <==
% \setlength\tabcolsep{1pt} % default value: 6pt
   \begin{small}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%\renewcommand{\arraystretch}{1.4} % Default value: 1 - only local changed within this table


    \begin{longtable}{lp{9cm}}
    \midrule[1pt]
    {Influencing Factor} & {Description}  \\ 
    \midrule[1pt]
   \textbf{Data}             &       \vspace*{0.15 cm}     \\
    \hspace{0.1cm} \textit{Data characteristics}     &        \\
\hspace{0.8cm} Data dependencies & Instability of data regarding their quality or quantity over time.  \\
\hspace{0.8cm} Data representation & Data formats, data structures, data types and further data representation aspects (e.g. data encoding). \\
\hspace{0.8cm} Data variety & Heterogeneity (i.e., formats, structures, types) of the data consumed.  \\
\hspace{0.8cm} Data volume & Quantity and rate at which data is coming into the pipeline.\vspace*{0.2 cm}  \\
    \hspace{0.1cm} \textit{Data management }    &        \\
\hspace{0.8cm} Data governance & Processes, policies, standards, and roles related to managing the data processed by a pipeline (e.g., data ownership, data accessibility, raw data storage). \\
\hspace{0.8cm} Data security & Degree to which data are protected during their transmission and processing. \\
\hspace{0.8cm} Metadata & Degree to which data consumed and processed are documented (e.g., data cataloge, data dictionary, data models, schemas). \vspace*{0.2 cm} \\ 
    
      \hspace{0.1cm} \textit{Data sources }    &        \\
    \hspace{0.8cm} Complexity & Number of data models and data sources a pipeline has to deal with including the degree of simplicity of merging the corresponding data (e.g., joinability). \\
\hspace{0.8cm} Reliability & Degree to which data sources are available, accessible and provide data of high quality.\vspace*{0.5 cm} \\
    
 
 
 
    
   \textbf{Development \& Deployment}             &       \vspace*{0.15 cm}     \\

\hspace{0.1cm}  \textit{Communication \&} \vspace{-0.08cm} \\ \hspace{0.1cm} \hspace*{1em}  \textit{information sharing} & \\
\hspace{0.8cm} Awareness & The perception of the pipeline as a coherent overall construct and the awareness and ability of knowledge exchange.  \\
\hspace{0.8cm} Requirements specifications & Completeness and level of detail regarding the specification and documentation of the pipeline (e.g., data transformation rules, processing requirements).\vspace*{0.2 cm}  \\

\hspace{0.1cm}  \textit{Personnel} & \\
\hspace{0.8cm} Domain knowledge & Entities knowledge and understanding about the domain underlying the data. \\
\hspace{0.8cm} Expertise & Background, experiences, technical knowledge, and quality awareness of entities.\vspace*{0.2 cm}  \\

\hspace{0.1cm}  \textit{Quality assurance} & \\
\hspace{0.8cm} Best practices & Code and configuration reviews, refactoring, canary processes and further best practices (e.g., use of control variables). \\
\hspace{0.8cm} Testing scope & Testing depth and space (e.g., test coverage, test cases). \vspace*{0.2 cm} \\

\hspace{0.1cm}  \textit{Training-serving skew} & \\
  \hspace{0.8cm} Code equality & Equality of software code between development and production (e.g., ported code, code paths, bugs). \\
\hspace{0.8cm} Data drift & Differences of the data between development and production (e.g., encodings, distribution). \vspace*{0.5 cm}\\
  
  
  
  
     \textbf{Infrastructure}             &       \vspace*{0.15 cm}     \\
  \hspace{0.1cm}  \textit{Serving environment} & \\
  
  \hspace{0.8cm} Hardware & Type and reliability of the hardware in production. \\
\hspace{0.8cm} Performance & Availability and manageability of the resources in production. \\
\hspace{0.8cm} Scalability & The capacity to change resources in size or scale. \vspace*{0.2 cm} \\
  
  
  
\hspace{0.1cm}  \textit{Tools \& technology} & \\
  \hspace{0.8cm} Appropriateness & Types (e.g., code/GUI-first, own solutions, propriety), maturity, flexibility and up-to-dateness of tools and technology. \\
\hspace{0.8cm} Compatibility & Ability of tools and technology (e..g, frameworks, platforms, libraries) to work together. \\
\hspace{0.8cm} Debugging capabilities & Availability and extent (i.e., level of detail) of opportunities (e.g., tools) to find and correct errors. \\
\hspace{0.8cm} Functionality & The scope of functions (e.g., advanced data operations, support of data management, engineering and validation) provided. \\
\hspace{0.8cm} Heterogeneity & Amount of different technologies and tools used.  \\
\hspace{0.8cm} Reliability & Degree to which tools and technologies are working correct (e.g., software quality, complexity). \\
\hspace{0.8cm} Usability & Availability, documentation and ease of use of APIs, libraries and tools. \vspace*{0.5 cm}\\





    \textbf{Life cycle management}             &       \vspace*{0.15 cm}     \\

\hspace{0.1cm}  \textit{Application management} & \\
\hspace{0.8cm} Configuration management & Version control and dependency management for code, libraries and configurations. \\
\hspace{0.8cm} Continuous integration \vspace{-0.08cm} & \multirow{2}{*}{Automation of providing new releases and changes.}   \\ \hspace*{1em} \hspace*{0.8cm} and deployment &  \\
\hspace{0.8cm} Workflow and \vspace{-0.08cm} & \multirow{2}{*}{Tools for managing the entire workflow of pipelines.}  \\ \hspace*{1em} \hspace*{0.8cm}  orchestration management \vspace*{0.2 cm} \\


\hspace{0.1cm}  \textit{Monitoring} & \\
\hspace{0.8cm} Application performance  \vspace{-0.08cm}  & \multirow{2}{*}{\shortstack[l]{Observing and logging the operational runtime of all \\ software components.}} \\
\hspace*{1em} \hspace*{0.8cm}monitoring & \\

\hspace{0.8cm} Data lineage & Observability of the data during all transformation steps including data versioning.\vspace*{0.5 cm} \\






    \textbf{Processing}             &       \vspace*{0.15 cm}     \\


\hspace{0.1cm}  \textit{Data flow architecture} & \\
\hspace{0.8cm} Complexity & Computational effort and pipeline complexity (e.g., transformation complexity). \\
\hspace{0.8cm} Dependencies & Dependencies between architectural components or processing steps. \\
\hspace{0.8cm} Modularization & Modularization of data pipeline components (e.g,, codes, APIs). \\
\hspace{0.8cm} Processing mode & Type of processing (e.g., batch, stream, distributed or parallel processing). \\
\hspace{0.8cm} Reproducibility & Degree to which processing is reproducable including aspects as caching and idempotency.  \\
\hspace{0.8cm} Sequence of data operations & Application order of data prepration and processing techniques.\vspace*{0.2 cm}  \\



\hspace{0.1cm}  \textit{Functionality} & \\
\hspace{0.8cm} Automation & Automation of data validation, handling, and providing corresponding guidance. \\
\hspace{0.8cm} Configuration & Configuration (e.g., parameters, settings) for processing data. \\
\hspace{0.8cm} Data cleaning & Treatment of data issues (e.g., modification or deletion). \vspace*{0.2 cm} \\


\hspace{0.1cm}  \textit{Software code} & \\
\hspace{0.8cm} Code quality & Quality and complexity of the code for processing data (e.g., dead code, duplicated code, language heterogeneity). \\
\hspace{0.8cm} Data type handling & Handling of data types (e.g., type casting, delimiter handling, encoding).\vspace*{0.2 cm}  \\



    \bottomrule
    \end{longtable}
   \end{small}



  

==> tables/tab-general_factors_all_rotated.tex <==
\begin{small}


\begin{landscape}
\begin{longtable}{lp{18 cm}}

    \midrule[1pt]
    {Influencing Factor} & {Description}  \\ 
    \midrule[1pt]
   \textbf{Data}             &       \vspace*{0.15 cm}     \\
    \hspace{0.1cm} \textit{Data characteristics}     &        \\
\hspace{0.8cm} Data dependencies & Instability of data regarding their quality or quantity over time.  \\
\hspace{0.8cm} Data representation & Data formats, data structures, data types and further data representation aspects (e.g. data encoding). \\
\hspace{0.8cm} Data variety & Heterogeneity (i.e., formats, structures, types) of the data consumed.  \\
\hspace{0.8cm} Data volume & Quantity and rate at which data is coming into the pipeline.\vspace*{0.2 cm}  \\
    \hspace{0.1cm} \textit{Data management }    &        \\
\hspace{0.8cm} Data governance & Processes, policies, standards, and roles related to managing the data processed by a pipeline (e.g., data ownership, data accessibility, raw data storage). \\
\hspace{0.8cm} Data security & Degree to which data are protected during their transmission and processing. \\
\hspace{0.8cm} Metadata & Degree to which data consumed and processed are documented (e.g., data cataloge, data dictionary, data models, schemas). \vspace*{0.2 cm} \\ 
    
      \hspace{0.1cm} \textit{Data sources }    &        \\
    \hspace{0.8cm} Complexity & Number of data models and data sources a pipeline has to deal with including the degree of simplicity of merging the corresponding data (e.g., joinability). \\
\hspace{0.8cm} Reliability & Degree to which data sources are available, accessible and provide data of high quality.\vspace*{0.5 cm} \\
    
 
 
 
    
   \textbf{Development \& Deployment}             &       \vspace*{0.15 cm}     \\

\hspace{0.1cm}  \textit{Communication \&} \vspace{-0.08cm} \\ \hspace{0.1cm} \hspace*{1em}  \textit{information sharing} & \\
\hspace{0.8cm} Awareness & The perception of the pipeline as a coherent overall construct and the awareness and ability of knowledge exchange.  \\
\hspace{0.8cm} Requirements specifications & Completeness and level of detail regarding the specification and documentation of the pipeline (e.g., data transformation rules, processing requirements).\vspace*{0.2 cm}  \\

\hspace{0.1cm}  \textit{Personnel} & \\
\hspace{0.8cm} Domain knowledge & Entities knowledge and understanding about the domain underlying the data. \\
\hspace{0.8cm} Expertise & Background, experiences, technical knowledge, and quality awareness of entities.\vspace*{0.2 cm}  \\

\hspace{0.1cm}  \textit{Quality assurance} & \\
\hspace{0.8cm} Best practices & Code and configuration reviews, refactoring, canary processes and further best practices (e.g., use of control variables). \\
\hspace{0.8cm} Testing scope & Testing depth and space (e.g., test coverage, test cases). \vspace*{0.2 cm} \\

\hspace{0.1cm}  \textit{Training-serving skew} & \\
  \hspace{0.8cm} Code equality & Equality of software code between development and production (e.g., ported code, code paths, bugs). \\
\hspace{0.8cm} Data drift & Differences of the data between development and production (e.g., encodings, distribution). \vspace*{0.5 cm}\\
  
  
  
  
     \textbf{Infrastructure}             &       \vspace*{0.15 cm}     \\
  \hspace{0.1cm}  \textit{Serving environment} & \\
  
  \hspace{0.8cm} Hardware & Type and reliability of the hardware in production. \\
\hspace{0.8cm} Performance & Availability and manageability of the resources in production. \\
\hspace{0.8cm} Scalability & The capacity to change resources in size or scale. \vspace*{0.2 cm} \\
  
  
  
\hspace{0.1cm}  \textit{Tools \& technology} & \\
  \hspace{0.8cm} Appropriateness & Types (e.g., code/GUI-first, own solutions, propriety), maturity, flexibility and up-to-dateness of tools and technology. \\
\hspace{0.8cm} Compatibility & Ability of tools and technology (e..g, frameworks, platforms, libraries) to work together. \\
\hspace{0.8cm} Debugging capabilities & Availability and extent (i.e., level of detail) of opportunities (e.g., tools) to find and correct errors. \\
\hspace{0.8cm} Functionality & The scope of functions (e.g., advanced data operations, support of data management, engineering and validation) provided. \\
\hspace{0.8cm} Heterogeneity & Amount of different technologies and tools used.  \\
\hspace{0.8cm} Reliability & Degree to which tools and technologies are working correct (e.g., software quality, complexity). \\
\hspace{0.8cm} Usability & Availability, documentation and ease of use of APIs, libraries and tools. \vspace*{0.5 cm}\\





    \textbf{Life cycle management}             &       \vspace*{0.15 cm}     \\

\hspace{0.1cm}  \textit{Application management} & \\
\hspace{0.8cm} Configuration management & Version control and dependency management for code, libraries and configurations. \\
\hspace{0.8cm} Continuous integration \vspace{-0.08cm} & \multirow{2}{*}{Automation of providing new releases and changes.}   \\ \hspace*{1em} \hspace*{0.8cm} and deployment &  \\
\hspace{0.8cm} Workflow and \vspace{-0.08cm} & \multirow{2}{*}{Tools for managing the entire workflow of pipelines.}  \\ \hspace*{1em} \hspace*{0.8cm}  orchestration management \vspace*{0.2 cm} \\


\hspace{0.1cm}  \textit{Monitoring} & \\
\hspace{0.8cm} Application performance  \vspace{-0.08cm}  & \multirow{2}{*}{\shortstack[l]{Observing and logging the operational runtime of all \\ software components.}} \\
\hspace*{1em} \hspace*{0.8cm}monitoring & \\

\hspace{0.8cm} Data lineage & Observability of the data during all transformation steps including data versioning.\vspace*{0.5 cm} \\






    \textbf{Processing}             &       \vspace*{0.15 cm}     \\


\hspace{0.1cm}  \textit{Data flow architecture} & \\
\hspace{0.8cm} Complexity & Computational effort and pipeline complexity (e.g., transformation complexity). \\
\hspace{0.8cm} Dependencies & Dependencies between architectural components or processing steps. \\
\hspace{0.8cm} Modularization & Modularization of data pipeline components (e.g,, codes, APIs). \\
\hspace{0.8cm} Processing mode & Type of processing (e.g., batch, stream, distributed or parallel processing). \\
\hspace{0.8cm} Reproducibility & Degree to which processing is reproducable including aspects as caching and idempotency.  \\
\hspace{0.8cm} Sequence of data operations & Application order of data prepration and processing techniques.\vspace*{0.2 cm}  \\



\hspace{0.1cm}  \textit{Functionality} & \\
\hspace{0.8cm} Automation & Automation of data validation, handling, and providing corresponding guidance. \\
\hspace{0.8cm} Configuration & Configuration (e.g., parameters, settings) for processing data. \\
\hspace{0.8cm} Data cleaning & Treatment of data issues (e.g., modification or deletion). \vspace*{0.2 cm} \\


\hspace{0.1cm}  \textit{Software code} & \\
\hspace{0.8cm} Code quality & Quality and complexity of the code for processing data (e.g., dead code, duplicated code, language heterogeneity). \\
\hspace{0.8cm} Data type handling & Handling of data types (e.g., type casting, delimiter handling, encoding).\vspace*{0.2 cm}  \\



    \bottomrule
    
\end{longtable}
\end{landscape}



   \end{small}



  
